AssemState: Manual and Physical-State-Guided Reasoning for Zero-shot Furniture Assembly

Multimodal large language models (MLLMs) have made significant progress in visual understanding, but precise 3D spatial reasoning integrated with physical environment remains difficult. Furniture assembly requires not only recovering step-level operations from diagrammatic manuals, but also translating semantic attachment relations into 6D pose updates that enable parts to physically interact with the environment and previously assembled components. To study this problem, we propose AssemState, a zero-shot framework for manual and physical-state-guided furniture assembly. It firstly employs anchor-guided boundary assembly states to decompose manual pages into single-part operations and recover an assembly-tree. Then, it uses iterative after-state feedback refinement to guide successive (SE(3)) updates and corrections, and validates their physical plausibility through simulation-based release tests. Experiments show that compared with the strongest prior baseline, AssemState improves F1 from 38.58\% to 62.80\% and Tree Exact Match from 28.24\% to 53.92\% for assembly-tree recovery. On 243 independently evaluated part-level operations, our proposed iterative refinement improves judge-accepted operations from 0 to 5.3\% and reduces mean Chamfer distance from 5.4111 to 1.7744. However, visually plausible candidate poses may still suffer from collision, floating, mirror-orientation errors, incomplete seating, and wrong-side attachment. These results show that AssemState improves operation-structure recovery and selected local pose metrics, while MLLMs remain limited for spatial relationship reasoning.

==> latex/sec/Limitations.tex <==
% \section{Limitations}

% Our evaluation is intentionally narrower than a full autonomous furniture-assembly system. First, the manual-side benchmark conditions on precomputed numbered step masks that highlight step-associated parts. The current materials document how these masks are consumed but do not evaluate their upstream construction; the assembly-tree results should therefore be interpreted as \emph{step-mask-conditioned structure recovery}, not raw-PDF-to-tree inference.

% Second, the pose benchmark isolates current-operation spatial reasoning. The correct current operation and preceding assembly state are provided, each operation is scored independently, and ground-truth pose is used only for scoring and post-scoring state reset. We therefore do not measure error propagation from the predicted assembly tree through a no-rescue end-to-end rollout.

% Third, judge acceptance is a model-based diagnostic rather than a human-validated ground-truth success label. We use it as a proxy for visible contact-level consistency and report geometric and simulation metrics alongside it. The strict PA@0.01 metric remains zero for all evaluated settings, and release-stability improvements are not uniform across backbones. These results limit our claim to improved structure recovery and selected local pose diagnostics, rather than reliable contact-accurate or physically executable assembly.


==> latex/sec/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% Filled for the AssemState workshop submission.

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state claims that are supported by the reported pose, geometry, and contact-consistency evaluations, with the scope limited to the evaluated furniture-assembly setting.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper's failure analysis and appendix describe important limitations, including oracle state-reset assumptions, simulation-only evaluation, and the limitations of the model-based judge.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not present theoretical results requiring assumptions or formal proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNo{}
    \item[] Justification: The paper documents the main protocol and metrics, but the complete historical judge prompts, aggregate API identifiers, and some experiment records are unavailable for exact reproduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: The current submission does not provide a complete public release of the code and data with instructions sufficient to reproduce all reported results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerNo{}
    \item[] Justification: Some data-split, per-table model, simulator, and API details needed to reproduce every experiment are not fully specified in the current version.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: The reported results do not include error bars, confidence intervals, or repeated-run significance analyses.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: The paper does not report the CPU/GPU configuration, memory, execution time, or API cost required for each experiment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work is presented as research on furniture-assembly reasoning and does not intentionally collect sensitive personal data or deploy a high-risk decision system; the authors should still follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{}
    \item[] Justification: The current paper does not explicitly discuss both potential benefits and risks, such as useful assembly assistance versus incorrect or unsafe assembly decisions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The submission does not release a high-risk model or dataset requiring controlled-release safeguards.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNo{}
    \item[] Justification: Existing manuals, meshes, datasets, simulators, and model services are cited or used, but their versions, licenses, and terms of use are not fully enumerated in the current submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The current submission does not introduce or release a new dataset, model checkpoint, code package, or other asset requiring accompanying asset documentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The experiments do not involve crowdsourcing or human-subject participants.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: No human-subject research or participant data are used, so IRB approval is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}
    \item[] Justification: LLMs are core experimental components: GPT-5 and Claude Haiku 4.5 are used for the reasoning pipeline and model-based judge acceptance evaluation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> latex/sec/test.tex <==
\section{Introduction}

Diagrammatic assembly manuals provide a natural source of procedural
knowledge for furniture assembly, specifying the parts, operation order,
and attachment relations required to construct a finished object.
Converting such manuals into machine-interpretable assembly instructions
could reduce the need for furniture-specific programming and
demonstration. However, this requires more than recognizing parts or
describing individual manual pages. An assembly system must recover the
operation structure across pages and translate each semantic attachment
relation into an explicitly parameterized spatial update that can be
applied to the evolving assembly state.

This problem presents two central challenges. First, manual pages and
part-level operations are not necessarily aligned: one page may contain
multiple attachments, visually similar parts may be interchangeable, and
the fixed subassembly changes as assembly progresses. We therefore define
an \emph{atomic operation} as a single-part attachment specification
containing the moving part, current fixed subassembly, attachment
relation, and pose hint. Recovering these operations requires maintaining
part identity and structural consistency across manual pages. Second, a
semantic instruction such as attaching a leg to a panel does not uniquely
determine the corresponding 6D pose. The model must reason about the
attachment side, insertion direction, mirror orientation, contact state,
and collision relative to the current subassembly. A pose that appears
plausible from one view may consequently remain geometrically or
physically invalid.

Existing datasets and environments, including IKEA-Manual, IAW, IKEA
Manuals at Work, IKEA Environment, and FurnitureBench, provide important
resources for studying manual understanding and furniture assembly
\cite{Wang2022IKEAManual,Zhang2023IAW,Liu2024IKEAManualsAtWork,
Lee2019IKEAEnv,Heo2023FurnitureBench}. Manual2Skill uses vision-language
models to recover hierarchical assembly graphs and combines them with
pose estimation and motion planning \cite{Tie2025Manual2Skill}, while
Manual2Skill++ introduces connector-aware representations for
fine-grained assembly relations \cite{Tie2025Manual2SkillPP}. A related
line of work studies language-guided 6D object rearrangement
\cite{baik2026textguided}. These methods establish the value of manuals
and visual-language reasoning for assembly, but they do not jointly
evaluate whether general-purpose multimodal large language models
(MLLMs) can convert diagrammatic manuals into structured part-level
operations and subsequently infer state-conditioned 6D pose updates
without a target pose or target image.

To study these capabilities, we present \textbf{FurniReason}, a zero-shot
framework that considers two complementary subtasks:
\emph{manual-to-operation generation} and
\emph{target-free 6D pose reasoning}. FurniReason implements these
subtasks with a manual reasoning module and a pose reasoning module.
The manual reasoning module grounds visually observed parts in the
manual and uses boundary-state anchors to align manual steps with the
evolving assembly state. It represents each atomic operation as
$a_k=(\mathcal{P}_{k,\mathrm{moving}},
\mathcal{P}_{k,\mathrm{fix}},r_k,h_k)$, explicitly specifying the moving
part, fixed subassembly, attachment relation, and pose hint. This
structured representation provides an interface between manual
understanding and downstream spatial reasoning.

The pose reasoning module translates each operation into an explicitly
parameterized $SE(3)$ update conditioned on the current assembly state.
Rather than relying on a single direct pose prediction, FurniReason
proposes a candidate update, applies it to the moving part, and renders
the resulting after-state from multiple views. An MLLM then diagnoses
contact and alignment errors, including wrong-side attachment, mirror
orientation, floating, incomplete seating, and collision, and produces
a constrained corrective $SE(3)$ update. Repeating this
render--diagnose--correct process converts implicit 3D reasoning into
multi-view visual inspection, for which current MLLMs provide stronger
visual priors.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{fig/overall2.png}
    \caption{\textbf{Overview of FurniReason.}
    (a) The manual reasoning module converts diagrammatic manuals into
    structured part-level operations and an assembly tree.
    (b) The pose reasoning module applies, renders, diagnoses, and
    iteratively refines state-conditioned 6D pose updates without a
    target pose or target image.}
    \label{fig:overall}
\end{figure}

Experiments show a clear difference between operation-structure recovery
and precise pose reasoning. For manual-to-operation generation,
FurniReason improves F1 from 38.58\% to 62.80\% and Tree Exact Match
from 28.24\% to 53.92\% over Manual2Skill++. We evaluate pose reasoning
on 55 correct-tree cases comprising 243 atomic operations, with each
operation evaluated independently from a ground-truth preceding assembly
state. With GPT-5, iterative refinement increases judge-accepted
operations from 0 to 5.3\% and reduces mean Chamfer distance from 5.4111
to 1.7744. However, all evaluated settings obtain zero PA@0.01, and
release stability does not improve consistently across MLLM backbones.
These results indicate that structured feedback improves selected
contact and geometric metrics, while current general-purpose MLLMs
remain unreliable for contact-accurate and physically executable
furniture assembly.

Our contributions are threefold:
(1) we formulate manual-guided furniture assembly as two complementary
zero-shot reasoning subtasks connected by a structured part-level
operation representation;
(2) we introduce an MLLM-based framework that combines boundary-state
anchoring for manual-to-operation generation with multi-view
render--diagnose--correct refinement for state-conditioned 6D pose
reasoning; and
(3) we provide an empirical analysis showing that MLLMs can improve
assembly-tree recovery and selected local pose metrics, while revealing
a substantial gap between visual plausibility, contact correctness,
strict pose accuracy, and simulation-based stability.
